Toward a Scalable Census of Dashboard Designs in the Wild: A Case Study with Tableau Public

Dashboards remain ubiquitous artifacts for presenting or reasoning with data across different domains. Yet, there has been little work that provides a quantifiable, systematic, and descriptive overview of dashboard designs at scale. We propose a schematic representation of dashboard designs as node-link graphs to better understand their spatial and interactive structures. We apply our approach to a dataset of 25,620 dashboards curated from Tableau Public to provide a descriptive overview of the core building blocks of dashboards in the wild and derive common dashboard design patterns. To guide future research, we make our dashboard corpus publicly available and discuss its application toward the development of dashboard design tools.

==> sections/archive/03-xx-Generalizability.tex <==
\subsection{Generalizability of the Representation}
\vidya{this subsection feels like it's overselling the paper before we go into the details of our method. Feels more like something that goes into the discussion to motivate people to explore the dataset for future research.}
% \arjun{I still get thrown off by this section as it gets into generalizability before describing what we did. Will be taking a shot at moving it down to limitations.}
% \leilani{The Previous Section 3.3 seemed like it was trying to speak to the generalizability and value of the schematic representation. I tried to address the comments in the previous version of that section by rewriting it. Feel free to reinstate the old version if this is off the mark.}

Our proposed schematic representation of dashboards is based solely on the constituent elements of dashboards and is thus agnostic to \emph{how} these elements were created. Further, this representation provides sufficient breadth to capture a wide range of design elements, from any type of visualization and text element to even non-visualization elements such as web pages. As a result, our schematic representation can capture the core elements of \emph{any} existing dashboard, whether this dashboard is specified programmatically using visualization languages, manually using graphic design tools, or automatically through recommendation systems. The value of this representation lies in how it provides a consistent \emph{intermediary representation} for dashboards that transcends individual tools. With a single representation, we can capture and analyze virtually any existing dashboard design, enabling our community to develop future corpora not as isolated islands but as inter-operable and comparable datasets amenable to rich meta-analysis.

In addition to its broad applicability, this schematic representation can easily be programmed for \emph{scalable} analysis of dashboard designs. It is straightforward to map the core elements of our representation to their counterparts within existing visualization languages and tools, as alluded to in Figure~\ref{fig:all-examples}. For example, one can map visualizations in Vega-Lite to chart blocks in our representation by extracting corresponding encoding sets from the underlying Vega-Lite specification. Similarly, one can write scripts to map Tableau workbooks into our proposed adjacency and interaction graphs. The resulting graphs can then be analyzed at scale using existing graph analysis, clustering, and summarization techniques, as we will show in the following section.

% >>>>Old Version:
% \subsection{Scaling Dashboard Analysis}
% \ana{I felt that this needed to be said specifically in this section so I gave it a go}.
% \arjun{With the new Figure 1 and updated text in 3.1 and 3.2 we might be able to remove this section and just expand what we have in the limitations section now. Need to revisit this later.}\michael{I think the stuff about ``well you could use CV and just look at the raster'' should go in either 3.1 or 2.3 (\cite{battle2018beagle,davila2021survey,poco2017,poco2018,prasad2007classifying,savva2011} all good refs). Stuff about ``not deriving frameworks'' not clear to me in the current section, but could be put added as context/explanation in either the intro or in 2.1}

% A consistent schematic representation of dashboard design  can scale analysis by serving as an intermediary between an initial specification and a design space resulting from a corpora of dashboards. There are many ways to do so. One approach to abstract the programmatic specifications for dashboards from their specification language. For example, dashboards created using Tableau, Shiny, Dash, or a D3/Vega-lite are all specified in different ways but could be compared if those low-level specifications are translated to our proposed blocks and connections schematic representation. Comparisons can occur within corpora, for example analyzing all dashboards created by Shiny,  or between corpora. When the initial specifications are not easily available, it may be possible to use other techniques, such as image segmentation~\ana{Add refs, I think Vidya had some}, to derive blocks and connections (spatial connections at a minimum).

% Regardless of the method used, the adjacency and interaction graphs that result from this effort can be analyzed at scale using existing graph analysis and clustering techniques, as well as descriptive statistics. Importantly, this approach is not intended to supplant approaches for deriving frameworks or design spaces, but instead provide a mechanism for leveraging them at scale to understand both the prevalence and scope of dashboard design in the wild. \ana{I feel like that last sentence sounds too defensive.}

==> sections/archive/xx-analysis.tex <==
\section{Analysis Results and Interpretation}
\label{sec:analysis-results}

In this section, we describe the  common dashboard design components and patterns revealed from the analysis of 25,620 Tableau Public dashboards. We organize our findings as responses to different design questions that we posed during the analysis.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/quant-results-combined.pdf}
    \caption{Summary statistics for (A) distribution of block types across dashboards and (B) distribution of interactive connection types across dashboards.}
    \label{fig:block-summary}
\end{figure*}

\subsection{Quantifying Dashboard Design}

\subsubsection{What are dashboards composed of?}\label{subsec:dash_composition}

We identified a total of 250,794 blocks across the 25,620 dashboards. The number of blocks per dashboard ranged from a minimum of 2 up to a maximum of 267, with a median of 8 and a mode of 4.  We observed that 121,068 out of 250,794 blocks (49\%) were {\charts}, followed by 53,267 {\textTmp} blocks (21\%), and subsequently {\filter} (36,472 or 15\%), {\legend} (22,446 or 9\%), and {\multimedia} (17541 or 7\%). We note the importance and centrality of text and charts as the building blocks of dashboards: together, over 70\% of the blocks in our analysis were one of these two block types.
Figure~\ref{fig:block-summary}A shows these results in detail.

For the {\chart} block type we also examined the distribution of visualization types across dashboards. We found that bar charts were the most common visualization type, appearing in 15,392 out of 25,620 (60\%) dashboards. Next most common were line charts (n=6,524; 25\%), maps (n=6,454; 25\%), and finally tables (n=6,154; 24\%). There were also instances of more specialized visualizations such as sankey diagrams and waterfall charts, but these were present in only 116 dashboards ($<$0.5\%). See Figure~\ref{fig:cluster_summary_stats} for summarized results of chart type information across clusters. This information points to many dashboards in our corpus representing a combination of simple charts (like bar charts) and a smaller set of more sophisticated dashboard designs.

\subsubsection{Is interactivity common in dashboards?}\label{subsec:dash_interaction}

Complementing our analysis of the visual components of dashboards, we also analyzed the connections between blocks to understand what types of interactions dashboards commonly support.
Note that we refer to a dashboard as \emph{interactive} if clicking on one block results in a visual change (e.g., filtering, brushing, updating fields) in another block, as opposed to other forms of interactivity that only involve individual blocks (e.g., hovering over a point in a single chart to generate a tooltip).

\vspace{0.5mm}
\noindent\textbf{Incidence of Interaction Connections.}
We found that 19,304 of the 25,620 dashboards in our corpus (75\%) were interactive and that their design patterns varied considerably.
The number of interaction connections between blocks ranged from 1 (e.g., a filter acting as a control for a single chart) to 992, with a median of 6 and mode of just 2 interaction connections in a dashboard. Recall that a single block can be the source or target of multiple interactions. The maximum possible interaction connections in a Tableau dashboard is bounded by  \begin{math}(\charts-1 + \legend + \filters) * \charts\end{math}. On average 58\% of the possible interactions between nodes were realized with a median of 50\% and mode of 100\%, suggesting that when authors add interactions, they do so to a great extent. We examined outlying instances with many interaction connections and found that in these dashboards, individual marks are configured to act as filters or selectors for other charts.

\vspace{0.5mm}
\noindent\textbf{Types of Interactions Observed.}
Of the three Tableau supported block interaction connections, {\filter}$\rightarrow${\chart} was most common with 13,228 out of the 19,304 dashboards (69\%) supporting this style of interaction, followed by {\chart}$\rightarrow${\chart} (46\% of dashboards) and {\legend}$\rightarrow${\chart} (43\% of dashboards). These results are summarized in Figure~\ref{fig:block-summary}B.

\vspace{0.5mm}
\noindent\textbf{Interactive Versus Non-Interactive Dashboard Structure.}
Lastly, we examined whether there were any notable differences in the visual components of these interactive dashboards compared to the other 6,316 non-interactive dashboards in our corpus.
%
As shown in Figure~\ref{fig:block-summary}A, besides the expected observation of interactive dashboards being comparably block dense (because of the {\filter} and {\legend} blocks added to facilitate interaction), \emph{we did not observe any notable differences} in the distributions of block types between interactive and static dashboards.
To check if the choice of visualizations influenced interactivity, we also compared the distributions of the 26,229 {\charts} in the static dashboards to the 94,839 {\charts} in the interactive dashboards.
Again, we did not observe any salient differences between the two groups.

The number and types of blocks in a dashboard directly affects the total number and types of interaction connections that we can surface. Our analysis shows that for authors of even comparatively simple dashboard designs, interactivity is an important aspect of exploring or communicating their data. More complex dashboard designs reveal intricate and nuanced examinations of data, but the relatively low number of examples suggests that a greater level of interactivity is either undesired or unachieved by the majority of dashboard authors.

\subsubsection{What are common spatial arrangements?}\label{subsec:dash_spatial}

In addition to analyses of the properties of individual blocks and interactivity between blocks, we also explored spatial relationships between blocks. 
Specifically, for the 25,620 dashboards, we analyzed the adjacency graphs to identify potential design patterns around dashboard layouts.
The graphs had 2-267 nodes (median 8, mode: 4) and 0-4926 edges (median: 11, mode: 3).
For each graph, we extracted the list of all maximal cliques, capturing the block type for each node in a clique (e.g., \{\chart$-$\chart$-$\chart\}, \{\chart$-$\filter\}, \{\multimedia\}).
Aggregating these maximal clique patterns across all graphs, we found a total of 1,430 unique blocks patterns. The smallest size cliques contained just 2 blocks and the largest contained 60, the median clique size was 9.  The most frequently occurring clique patterns contained just two blocks, typically including a {\chart} and one of the other block types; a summary of the most  frequently occurring patterns is in Figure~\ref{fig:clique-summary}A.

\begin{figure}[t!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/clique-summary.pdf}
    \vspace{-2mm}
    \caption{Frequently occurring clique patterns from the adjacency graph analysis. Nodes map to different block types including {\chart}, {\textTmp}, {\filter}, {\legend}, and {\multimedia}.}
    \label{fig:clique-summary}
\end{figure}

Focusing on {\chart} blocks specifically, we can also examine the creation of juxtaposed views. Of all 1,430 unique clique patterns, more than half (n=747) contained a spatial arrangement of two or more {\charts}; we list the five most frequently occurring clique patterns in Figure~\ref{fig:clique-summary}B. The most dominant patterns are cliques containing only {\chart} block types, varying in size from 2 to 4. When two {\chart} blocks occur with other blocks, it was more common for those other blocks to be a {\textTmp} or {\multimedia} block.

Collectively, the clique analysis reveals that certain design strategies are repeated across dashboards. As with prior analysis, the results emphasize simpler dashboard designs, but, reiterate that authors do experiment with more complex designs that mix block types.


\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/cluster-table-mc3.pdf}
    \vspace{-4mm}
    \caption{Select statistical summaries for the clusters in \autoref{fig:tsne_clusters}. Note many visualization types are ubiquitous within particular clusters. The ``Other'' visualizations that are dominant in clusters \protect\cluster{1},\protect\cluster{2},\protect\cluster{3},\protect\cluster{4},\protect\cluster{5}, and \protect\cluster{6} are radial charts, histograms, area charts, treemaps, and dotplots, respectively.}
    \vspace{-5mm}
    \label{fig:cluster_summary_stats}
\end{figure*}

\subsection{Dashboard Design Clusters}

Our prior analysis points to heterogeneities in dashboard design in terms of both visual and interaction design. To capture these differences, we perform a cluster analysis of our corpus.

\subsubsection{Cluster Descriptive Statistics}
A total of 10,187 dashboards (40\%) produced a set of 27 clusters. The remaining 60\% of dashboards could not be assigned to any one single cluster. There are various reasons why a dashboard does not become part of a cluster; for example, highly bespoke and unique dashboard designs may not easily form part of any cluster, other dashboards may belong to multiple clusters and may not obviously belong in just one, and some dashboards may not have enough signal to cluster with anything. The choice of clustering parameters also affects the number of dashboards that form clusters. The resulting set of clusters represents both common and recurrent design patterns across the Tableau Public Repository. The membership of clusters ranged from 108 to 761 dashboards (recall the minimum cluster size supplied to HDBSCAN was 100, see Section~\ref{subsec:clusters}), with a median of 361 dashboards.  The number of impressions (see Section~\ref{subsec:dash_winnow}) is similar across clusters, ranging from 64 to 920 median impressions.

\vspace{0.5mm}
\noindent\textbf{Cluster Cohesiveness.} We compute the average silhouette scores to determine the cohesiveness of dashboards within a cluster; the silhouette score ranges from -1 to 1, with 1 indicating that all dashboards with a cluster are identical.  Small clusters tended to have higher silhouette scores compared to larger clusters, which implies that these smaller clusters have more homogeneous design patterns, whereas larger ones may capture more variety. This observation suggests that simply the number and variety of block and visualization types, rather than any specific design patterns,  may be a driver in the cluster analysis that results in the lower cohesiveness of large clusters.  Cluster \cluster{16} had both the greatest cluster cohesiveness (0.841) and impressions (median per dashboard is 920). However, on examination, the dashboards within the cluster seem to consist exclusively of combinations of line and bar {\chart} blocks without any interactivity.

\vspace{0.5mm}
\noindent\textbf{Diversity of Blocks and Connections.} We can further explore the composition of clusters relative to their block types and interaction connections.  We observed that clusters tended to organize themselves along an axis of interaction. Seven clusters (\cluster{10},\cluster{12} and \cluster{15}-\cluster{19}) representing 2,052 dashboards, had no interactivity at all. These non-interactive clusters tended to feature simple dashboard designs with few block types and generally had {\chart} blocks with just one visualization type (either bar, line, table, map, or scatter charts; an exception is cluster \cluster{16} which has both bar and line charts). As interactivity increases, the diversity of block types also increases, but not necessarily the diversity of visualization types. For example, dashboards in cluster \cluster{20} had both high interactivity in terms of actions and the near-ubiquitous presence of non-{\chart} blocks that permit interaction (\text,\filter,\legend,\multimedia), but little variety in visualization types (bar charts were ubiquitous, but other common chart types were absent).  Two notable exceptions are clusters \cluster{0} and \cluster{1} which have more interactivity \emph{and} a broad diversity of block and visualization types. 

\vspace{0.5mm}
\noindent\textbf{Compositions of Visualizations.} Finally, examining {\chart} blocks, we find that the majority of clusters prominently feature a single ubiquitous or near-ubiquitous visualization type. Most often, this visualization is a bar chart (clusters \cluster{16},\cluster{18}, and \cluster{20}-\cluster{26}), but we also observed clusters featuring primarily (or only) maps (\cluster{12},\cluster{13}), tables (\cluster{10},\cluster{11}), pie charts (\cluster{9}), and scatter plots (\cluster{8}) as their component visualizations. Commensurate with prior observations (see Sections~\ref{subsec:dash_composition} and~\ref{subsec:dash_spatial}), there are many potential explanations for these clusterings that center around chart type: for instance, a desire for simplicity and avoiding unnecessary visual complexity or limits and influence in tooling. However, other potential similarities within dashboards of similar chart types might reflect congruent analytical purposes (e.g., dashboards with line charts might be similar because they are dashboards of time series data and so have unifying desired affordances or expressiveness) or even reflect pedagogical or skill-sharing structures (for instance a ``lineage'' of dashboards built from similar models or off of similar tutorials, or even dashboard authors exploring single chart types in dashboards meant for learning rather than data communication).


\subsection{Qualitative Analysis of Dashboards}
\label{sec:qual}

We performed a qualitative analysis of a subset of 54 exemplar dashboards across all clusters. From this analysis, we generated a set of observed emergent themes in authoring practices across our exemplar dashboards.


\vspace{.5em}
\noindent{\textbf{Text and Context.}}
After {\charts}, {\textTmp} blocks were the most popular and were present in 15,629 out of the 25,620 dashboards (61\%). Members of six clusters (\cluster{15},\cluster{18},\cluster{20},\cluster{24},\cluster{25},\cluster{26}) represent 1,115 dashboards all having text elements. These {\textTmp} blocks are used to explain context, takeaways, or provide instructions on how to interact with or interpret the dashboard. We also observed examples of authors using text to alert viewers to idiosyncrasies or concerns about the data. 


\vspace{.5em}
\noindent{\textbf{Layout and Widget Placement.}} 
We observed recurring UI patterns when it came to the placement of blocks. Larger-sized views were usually placed at the top of the dashboard, with views of a similar visualization type and size placed next to one another. With respect to interactivity, we often observed a single ``control panel'' area containing all of the relevant filters and legends for a dashboard. These control panels were often in the periphery of the dashboard (e.g., Figure~\ref{fig:tsne_clusters}, \cluster{20}, which has an extensive control panel of filters on the right side). In contrast to the ``control panel'', another pattern of interactive dashboard interface was that of \textit{in situ} widgets. In this pattern, the filters were dispersed across the dashboard in a way that associated them with individual charts (e.g., a \filter is contained or otherwise adjacent as per Figure~\ref{fig:adjacency-scenarios} with the {\chart} that it uniquely impacts).

\vspace{.5em}
\noindent{\textbf{Mistakes and Violations:}} 
There was a heterogeneity of visual design and Tableau skill in our corpus, occasionally leading to dashboards that do not operate as assumed or as recommended by existing practices. For instance, two of the dashboards in our qualitative sample (within clusters \cluster{23} and \cluster{26}) reused categorical colors across multiple data columns, resulting in an ``inconsistent''~\cite{qu2017keeping} dashboard where the meaning of a particular color was ambiguous. These potential errors or oversights also occurred in the interaction design: for instance, we observed {\filter} blocks that seemed applicable to multiple charts in a dashboard but that would seem to only impact one chart. We also note that in many cases, the interactive \textit{affordances} of the dashboards were unclear and the interaction model we extracted in Figure~\ref{fig:feature-extraction}C was often helpful for us in our qualitative coding to identify interactions between blocks that we otherwise would have missed (e.g., that a {\legend} could be used to highlight or filter associated {\chart} blocks).

\vspace{.5em}
\noindent{\textbf{Personalization and Expression.}} Lastly, we observe diversity in the degree of customization and analytical goals of the dashboards in our corpus.
Some dashboards consisted of only basic pre-formatted charts or summary statistics while others contained a variety of views with extensive customization for both {\charts} and other blocks (e.g., custom fonts or styles for {\textTmp} blocks).
For instance, one dashboard in cluster \cluster{0} (Figure~\ref{fig:tsne_clusters}, \cluster{0}) was an infographic-style dashboard with a ``sketchy'' hand-drawn image, chart, and text style. 
% Others, however, relied on Tableau default designs (such as standard Tableau colors).
This heterogeneity extended also to analytical ``style'': we saw many different formats, from ``conventional'' monitoring dashboards of key metrics based on organizational or demographic data, to long and dense infographics and even some dashboards meant for pedagogy (e.g., to explain or illustrate particular features of Tableau).
